Full Iso-recursive Types

There are two well-known formulations of recursive types: iso-recursive and equi-recursive types. Abadi and Fiore [1996] have shown that iso- and equi-recursive types have the same expressive power. However, their encoding of equi-recursive types in terms of iso-recursive types requires explicit coercions. These coercions come with significant additional computational overhead, and complicate reasoning about the equivalence of the two formulations of recursive types. This paper proposes a generalization of iso-recursive types called full iso-recursive types. Full iso-recursive types allow encoding all programs with equi-recursive types without computational overhead. Instead of explicit term coercions, all type transformations are captured by computationally irrelevant casts, which can be erased at runtime without affecting the semantics of the program. Consequently, reasoning about the equivalence between the two approaches can be greatly simplified. We present a calculus called $\lambda^{\mu}_{Fi}$, which extends the simply typed lambda calculus (STLC) with full iso-recursive types. The $\lambda^{\mu}_{Fi}$ calculus is proved to be type sound, and shown to have the same expressive power as a calculus with equi-recursive types. We also extend our results to subtyping, and show that equi-recursive subtyping can be expressed in terms of iso-recursive subtyping with cast operators.

==> Makefile <==
## Add a new source ott-processed file foo as:  src/foo.ott.tex
##   reference as  pp/foo.tex

TEX_FILES=sections/calculus.tex \
	sections/introduction.tex \
	sections/metatheory.tex \
	sections/overview.tex \
	sections/related.tex \
	sections/subtyping.tex

FIG_DIR=figures

.DEFAULT_GOAL := main.pdf

ifneq (,$(findstring WSL, $(shell uname -r)))
    LATEXMK = latexmk.exe
else
    LATEXMK = latexmk
endif

##### OTT COMPILATION {{{ #####

OTT_FILE=rules/rules
OTT_SRC=${OTT_FILE}.ott
OTT_TEX=${OTT_FILE}.tex
OTT_FLAGS=-tex_wrap false

${OTT_TEX} : ${OTT_SRC}
	ott ${OTT_FLAGS} -i $< -o $@

##### }}} #####



.PHONY : main.pdf
main.pdf : main.tex base.bib ${OTT_TEX} ${TEX_FILES}
	$(LATEXMK) -pdf main.tex

.PHONY : all
all : main.pdf

.PHONY : open
open : main.pdf
	open main.pdf

rules : ${OTT_TEX}

.PHONY : clean
clean :
	$(LATEXMK) -C
	rm -rf main.bbl ${OTT_TEX}


==> README <==
## Abstract



There are two well-known formulations of recursive types: iso-recursive and   
equi-recursive types.
Abadi and Fiore [1996] have shown that
iso- and equi-recursive types have the same expressive power.
However, their encoding of equi-recursive types in terms of
iso-recursive types requires explicit coercions. These coercions come
with significant
additional computational overhead, and complicate reasoning
about the equivalence of the two formulations of recursive types.

This paper proposes a
generalization of iso-recursive types called full
iso-recursive types. Full iso-recursive types allow encoding
all programs with equi-recursive types without
computational overhead. Instead of explicit term coercions, all 
type transformations are captured by computationally
irrelevant casts, which can be erased at runtime without
affecting the semantics of the program. Consequently, reasoning about
the equivalence between the two approaches can be greatly simplified.
We present a calculus called $\lambda^{\mu}_{Fi}$, which extends the simply typed
lambda calculus (STLC) with full iso-recursive types. The $\lambda^{\mu}_{Fi}$
calculus is proved to be type sound, and shown to have the same
expressive power as a calculus with equi-recursive types.
We also extend our results to subtyping, and 
show that equi-recursive subtyping can
be expressed in terms of iso-recursive subtyping with cast operators.
